Morphence: Moving Target Defense Against Adversarial Examples

Robustness to adversarial examples of machine learning models remains an open topic of research. Attacks often succeed by repeatedly probing a fixed target model with adversarial examples purposely crafted to fool it. In this paper, we introduce Morphence, an approach that shifts the defense landscape by making a model a moving target against adversarial examples. By regularly moving the decision function of a model, Morphence makes it significantly challenging for repeated or correlated attacks to succeed. Morphence deploys a pool of models generated from a base model in a manner that introduces sufficient randomness when it responds to prediction queries. To ensure repeated or correlated attacks fail, the deployed pool of models automatically expires after a query budget is reached and the model pool is seamlessly replaced by a new model pool generated in advance. We evaluate Morphence on two benchmark image classification datasets (MNIST and CIFAR10) against five reference attacks (2 white-box and 3 black-box). In all cases, Morphence consistently outperforms the thus-far effective defense, adversarial training, even in the face of strong white-box attacks, while preserving accuracy on clean data.

==> related.tex <==
\section{Related Work}\label{sec: related}
We review related work along three lines: moving target defense, best-effort/empirical defense, and certified defense. We make more concrete comparisons \sysname{} and moving target defenses.

\textbf{Moving Target Defenses.}
Network and software security has leveraged numerous flavors of MTD including randomization of service ports and address space layout randomization. Recent work has explored MTD for defending adversarial examples.
Song et al.~\cite{fMTD19} proposed a fMTD where they create fork-models via independent perturbations of the base model and retrain them. Fork-models are updated periodically whenever the system is in an idle state. The input is sent to all models and the prediction label is decided by majority vote. \\
Sengupta et al. \cite{MTDeep19} proposed  MTDeep, which uses different DNN architectures (e.g., CNN, HRNN, MLP) in a manner that reduces transferability between model architectures using a measure called {\em differential immunity}. Through Bayesian Stackelberg game, MTDeep chooses a model to classify an input. Despite diverse model architectures, MTDeep suffers from a small model pool size.\\
Qian et al.~\cite{EI-MTD} propose EI-MTD, a defense that leverages the Bayesian Stackelberg game for dynamic scheduling of student models to serve prediction queries on resource-constrained edge devices. The student models are generated via differential distillation from an accurate teacher model that resides on the cloud. 


\textbf{Compared to EI-MTD~\cite{EI-MTD}}, \sysname{} avoids inheritance of adversarial training limitations by adversarially training a subset of student models instead of the base model. Unlike EI-MTD that results in lower accuracy on clean data after adversarial training, \sysname{}'s accuracy on clean data after adversarial training is much better since the accuracy penalty is not inherited by student models. Instead of adding regularization term during training, \sysname{} uses distinct transformed training data to retrain student models and preserve base model accuracy. Instead of the Bayesian Stackelberg game, \sysname{} uses the most confident model for prediction. 

\textbf{With respect to MTDeep~\cite{MTDeep19}}, \sysname{} expands the pool size regardless of the heterogeneity of individual models and uses average transferability rate to estimate attack transferability. On scheduling strategy, instead of Bayesian Stackelberg game \sysname{} uses the most confidence model. 

\textbf{Unlike fMTD~\cite{fMTD19}}, \sysname{} goes beyond retraining perturbed fork models and adversarially trains a subset of the model pool to harden the whole pool against adversarial example attacks. In addition, instead of majority vote, \sysname{} picks the most confident model for prediction. For pool renewal, instead of waiting when the system is idle, \sysname{} takes a rather safer and transparent approach and renews an expired pool seamlessly on-the-fly. \\
\textbf{Best-Effort Heuristic Defenses.}
In this class of defenses, several defense approaches have been proposed, most of which were subsequently broken \cite{Carlini-Breaking17,Carlini-BreakingUsenix17,Gradient-Masking18}. Many of the early attempts~\cite{Early-Defense14,Early-Defense15} to harden ML models (specially neural networks) provided only marginal robustness improvements against adversarial examples. In the following, we highlight these line of defenses. \\
{\em Defensive distillation} by Papernot et al.~\cite{distillation} is a strategy to distill knowledge from neural network as soft labels by smoothing the {\em softmax} layer of the original training data. It then uses the soft labels to train a second neural network that, by way of hidden knowledge transfer, would behave like the first neural network. The key insight is that by training to match the first network, one will hopefully avoid over-fitting against any of the training data. Defensive distillation was later broken by Carlini and Wagner~\cite{CW}.\\
{\em Adversarial training}~\cite{FGSM}: While effective against the class of adversarial examples a model is trained against, it fails to catch adversarial examples not used during adversarial training. Moreover, robustness comes at a cost of accuracy penalty on clean inputs.\\
{\em Data transformation approaches} such as compression~\cite{Compression17,Compression18}, augmentation~\cite{Augmentation17}, cropping~\cite{Cropping17}, and randomization~\cite{Rand15,Rand18} have also been proposed to thwart adversarial examples. While these lines of defenses are effective against attacks constructed without the knowledge of the transformation methods, all it takes an attacker to bypass such countermeasures is to employ novel data transformation methods. Similar to adversarial training these approaches also succeed at a cost of accuracy loss on clean data.\\
{\em Gradient masking approaches} (e.g., \cite{Thermo-Encode18,PixelDefend18}) are based on obscuring the gradient from a white-box adversary. However, Athalye et al.~\cite{Gradient-Masking18} later broke multiple gradient masking-based defenses.

\textbf{Certifiably Robust Defenses.}
Most best-effort defenses remain vulnerable because adaptive adversaries work around their defensive heuristics. 
In an attempt to  obtain a theoretically justified guarantee of robustness, certified defenses have been recently proposed~\cite{wong2018provable,raghunathan2020certified,lecuyer2019certified,RandomSmoothing19}. The key idea is to provide provable/certified robustness of ML models under attack.
Lecuyer et al.\cite{lecuyer2019certified} prove robustness lower bound with differential privacy using Laplacian and Gaussian noise after the first layer of a neural network. Li et al.~\cite{Certified-AdditiveNoise19} build on~\cite{lecuyer2019certified} to prove certifiable lower bound using Renyi divergence. To stabilize the effect of Gaussian noise. Cohen et al.~\cite{RandomSmoothing19} propose randomized smoothing with Gaussian noise to guarantee adversarial robustness in $l_2$ norm by turning any classifier that performs well under Gaussian noise into a new classifier that is certifiably robust to adversarial perturbations under $l_2$ norm. 
